Towards Touch-to-Access Device Authentication Using Induced Body Electric Potentials

This paper presents TouchAuth, a new touch-to-access device authentication approach using induced body electric potentials (iBEPs) caused by the indoor ambient electric field that is mainly emitted from the building's electrical cabling. The design of TouchAuth is based on the electrostatics of iBEP generation and a resulting property, i.e., the iBEPs at two close locations on the same human body are similar, whereas those from different human bodies are distinct. Extensive experiments verify the above property and show that TouchAuth achieves high-profile receiver operating characteristics in implementing the touch-to-access policy. Our experiments also show that a range of possible interfering sources including appliances' electromagnetic emanations and noise injections into the power network do not affect the performance of TouchAuth. A key advantage of TouchAuth is that the iBEP sensing requires a simple analog-to-digital converter only, which is widely available on microcontrollers. Compared with existing approaches including intra-body communication and physiological sensing, TouchAuth is a low-cost, lightweight, and convenient approach for authorized users to access the smart objects found in indoor environments.

==> Makefile <==
DOC=touchauth

all: 
	pdflatex $(DOC).tex
	bibtex $(DOC)
	pdflatex $(DOC).tex
	pdflatex $(DOC).tex
	pdflatex $(DOC).tex

o:
	pdflatex $(DOC).tex

clean:
	rm -f $(DOC).blg $(DOC).log $(DOC).toc $(DOC).lot $(DOC).lof $(DOC).out $(DOC).ps $(DOC).aux $(DOC).zip comment.cut


publish:
	texdirflatten -1 -f touchauth.tex -o output --imgexts .pdf

dvi:
	#if [ ! -f dvimode ] ; \
	#then \
	#	echo "Entering dvimode" ; \
	#	echo "" > dvimode ; \
	#	sed -i '/\RequirePackage\[libertine\]{newtxmath}/c\\\RequirePackage\[italic\]{mathastext}' acmart.cls; \
	#fi;
	#latex -src-specials -halt-on-error $(DOC)
	pdflatex -synctex=1 -src-specials -interaction=nonstopmode $(DOC)

bib:
	bibtex $(DOC)

pdf:
	#if [ -f dvimode ] ; \
	#then \
	#	echo "Exiting pdfmode" ; \
	#	rm -f dvimode ; \
	#	sed -i '/\RequirePackage\[italic\]{mathastext}/c\\\RequirePackage\[libertine\]{newtxmath}' acmart.cls; \
	#fi;
	#latex $(DOC)
	#dvips -t letter $(DOC).dvi
	#ps2pdf $(DOC).ps
	pdflatex $(DOC)
	pdflatex $(DOC)

cleanall: clean
	find . -name '*-converted-to.pdf' -delete
	find . -name '*.fdb_latexmk' -delete
	find . -name '*~' -delete
	$(RM) $(PDF) *-converted-to.pdf

prepare:
	make all
	make clean
	cd figs && python pdf2eps.py
	make merge

merge:
ifeq ($(OS),Windows_NT)   
	unison . ..\..\Zhenyu\TouchAuth-revision
else
	unison ./ ../../Zhenyu/TouchAuth-revision
endif


drop:
	unison dropbox2 ~/research/wear-pair/mobicom-cameraready ~/Dropbox/Zhenyu/TouchAuth-revision


